NM-FlowGAN: Modeling sRGB Noise without Paired Images using a Hybrid Approach of Normalizing Flows and GAN

Modeling and synthesizing real sRGB noise is crucial for various low-level vision tasks, such as building datasets for training image denoising systems. The distribution of real sRGB noise is highly complex and affected by a multitude of factors, making its accurate modeling extremely challenging. Therefore, recent studies have proposed methods that employ data-driven generative models, such as Generative Adversarial Networks (GAN) and Normalizing Flows. These studies achieve more accurate modeling of sRGB noise compared to traditional noise modeling methods. However, there are performance limitations due to the inherent characteristics of each generative model. To address this issue, we propose NM-FlowGAN, a hybrid approach that exploits the strengths of both GAN and Normalizing Flows. We combine pixel-wise noise modeling networks based on Normalizing Flows and spatial correlation modeling networks based on GAN. Specifically, the pixel-wise noise modeling network leverages the high training stability of Normalizing Flows to capture noise characteristics that are affected by a multitude of factors, and the spatial correlation networks efficiently model pixel-to-pixel relationships. In particular, unlike recent methods that rely on paired noisy images, our method synthesizes noise using clean images and factors that affect noise characteristics, such as easily obtainable parameters like camera type and ISO settings, making it applicable to various fields where obtaining noisy-clean image pairs is not feasible. In our experiments, our NM-FlowGAN outperforms other baselines in the sRGB noise synthesis task. Moreover, the denoising neural network trained with synthesized image pairs from our model shows superior performance compared to other baselines. Our code is available at: \url{https://github.com/YoungJooHan/NM-FlowGAN}.

==> sec/table/table_kld_baselines.tex <==
\begin{table}[!bt]
\caption{
\textbf{KL divergence between synthesized noise and real noise calculated under various camera types.} \textbf{Bold} numbers indicate the best performance (lower is better), while \textit{underlined} numbers indicate the second best. $\dagger$ denotes the method of synthesizing sRGB noise with a paired noisy image, which is a more constrained approach that should be considered when interpreting this table.
}
\centering
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}
\scalebox{1.0}{
\begin{tabular}{c | ccccc | c }
\hline
\bf \textsc{Method} & \bf \textsc{G4} & \bf \textsc{GP} & \bf \textsc{IP} & \bf \textsc{N6} & \bf \textsc{S6} & \bf \textsc{ALL} \\
\hline
AWGN                                    & 0.067 & 0.114 & 0.056 & 0.147 & 0.084	 & 0.086        \\
Heteroscedastic                         & 0.072 & 0.139 & 0.058 & 0.133 & 0.082	 & 0.078 	    \\
C2N~\cite{c2n}                          & 0.230 & 0.446 & 0.117 & 0.240 & 0.682 & 0.388	    \\
sRGBFlow~\cite{srgb_flow}               & 0.042 & 0.067 & 0.039 & 0.053 & 0.044	 & 0.048 	    \\
NeCA-W~\cite{neca}                        & 0.089 & 0.087 & 0.045 & 0.085 & 0.072	 & 0.071        \\ 
NeCA-W$^\dagger$~\cite{neca}                  & 0.061 & \underline{0.026} & 0.028 & 0.043 & 0.034	 & 0.034        \\ 
NAFlow$^\dagger$~\cite{naflow}                  & \textbf{0.019} & 0.068 & \textbf{0.013} & \underline{0.042} & \textbf{0.016}	 & \textbf{0.028}        \\ 
\hline
\textbf{Ours}                       & \underline{0.039} & \textbf{0.026} & \underline{0.017} & \textbf{0.041} & \underline{0.033}	 & \underline{0.028} 	    \\
\hline
\end{tabular}
}
\label{table:table_unknown}
\end{table}



==> sec/table/table_psnr_ssim_baselines.tex <==
\begin{table}[!bt]
\centering
\caption{
\textbf{Image denoising results on the SIDD benchmark dataset.} Each denoiser is trained on synthesized noisy-clean image pairs generated by each model. $^\dagger$ denotes the method of synthesizing sRGB noise with a paired noisy image, which is a more constrained approach that should be considered when interpreting this table. %Compared to denoisers trained on image pairs from other baselines, the denoisers trained on our synthesized noisy-clean image pairs achieve promising denoising performance.
}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{9pt}
\scalebox{1.0}{
\begin{tabular}{ ccc | cc }
\hline
&\bf \textbf{Method}& & \bf \textbf{PSNR}(dB) & \bf \textbf{SSIM} \\
\hline
&AWGN&                                    & 32.48 & 0.854        \\
&Heteroscedastic&                         & 32.13 & 0.843  	    \\
&C2N~\cite{c2n}&                          & 33.76 & 0.901    \\
&sRGBFlow~\cite{srgb_flow}&               & 34.74 & 0.912 	    \\
&NeCA-W~\cite{neca}&                        & 35.93 & 0.926          \\ 
&NeCA-W$^\dagger$~\cite{neca}&                        & 36.82 & 0.932          \\ 
&NAFlow$^\dagger$~\cite{naflow}&                        & 37.22 & 0.935          \\ 
\hline
&\textbf{Ours}&                         & \textbf{37.04} & \textbf{0.932}  	    \\
\hline
&Real Noisy&                      & 37.73 & 0.941  \\
\hline
\end{tabular}
}
\label{table:table_psnr_ssim_baselines}
\end{table}


